Near Optimal Compressed Sensing of a Class of Sparse Low-Rank Matrices via Sparse Power Factorization

Compressed sensing of simultaneously sparse and low-rank matrices enables recovery of sparse signals from a few linear measurements of their bilinear form. One important question is how many measurements are needed for a stable reconstruction in the presence of measurement noise. Unlike conventional compressed sensing for sparse vectors, where convex relaxation via the $\ell_1$-norm achieves near optimal performance, for compressed sensing of sparse low-rank matrices, it has been shown recently Oymak et al. that convex programmings using the nuclear norm and the mixed norm are highly suboptimal even in the noise-free scenario. We propose an alternating minimization algorithm called sparse power factorization (SPF) for compressed sensing of sparse rank-one matrices. For a class of signals whose sparse representation coefficients are fast-decaying, SPF achieves stable recovery of the rank-1 matrix formed by their outer product and requires number of measurements within a logarithmic factor of the information-theoretic fundamental limit. For the recovery of general sparse low-rank matrices, we propose subspace-concatenated SPF (SCSPF), which has analogous near optimal performance guarantees to SPF in the rank-1 case. Numerical results show that SPF and SCSPF empirically outperform convex programmings using the best known combinations of mixed norm and nuclear norm.

==> RDv.tex <==

In this appendix we prove a rate-distortion lower bound for the one-dimensional uniform random subspace with respect to the mean-square error loss between projection matrices. On a related note, we remark that the rate-distortion function of uniform distribution on the sphere
 with respect to the mean-square error has been obtained in \cite{Harremoes09,Harremoes10} in a parametric form.

\begin{theorem}
	Let $v$ be uniformly distributed on the complex unit sphere $\bbS^{2n-1}$.
	Let $E_n = \{uu^*: u \in \bbS^{2n-1}\}$ denote the collection of all $n \times n$ rank-one Hermitian matrices.
	Let $\log^+ \triangleq \max\{\log, 0\}$.
%	Then there is an absolute constant $C < XXX$, such that
	Then for any $n \geq 2$ and any $0 < D < 2$,
	\begin{align}
%	\inf_{P_{\hv|v}: \Expect \|v-\hv\|_2^2 \leq D} I(v;\hv)  \geq & ~ 	n \log^+ \frac{1}{D+\frac{D^2}{4} + \frac{1}{n}\big(1-\frac{D}{2}\big)^2}, 	\label{eq:RDv}\\
	\inf_{P_{\hv\hv^*|vv^*}: \Expect \|vv^*-\hv\hv^*\|_{\mathrm{F}}^2 \leq D} I(vv;\hv\hv^*)  \geq & ~ 	(n-1) \log^+ \frac{1}{6D} - 3.5, 	\label{eq:RDvv}
\end{align}
where the infimum is taken over all probability transition kernels from $E_n$ to itself.
	\label{thm:RDv}
\end{theorem}
\begin{remark}
Therefore the lower bound in \prettyref{thm:RDv} is in fact asymptotically sharp in the low-distortion regime, and the rate-distortion function on the left-hand side of \prettyref{eq:RDvv} is in fact $(n-1) \log \frac{1}{D}(1+o(1))$ when $D \to 0$, since a matching upper bound can be obtained by quantizion and using the covering number bound of the Grassmannian manifold \cite{Szarek82}. To interpret the pre-log factor $n-1$, we recall that the low-distortion asymtotics of the rate-distortion function is known \cite{KD94} to be: $R_X(D) = \frac{d(X)}{2} \log \frac{1}{D}(1+o(1))$, where the distortion is mean-square error and $d(X)$ is the \emph{information dimension} of the random vector $X$ \cite{renyi}, which, in the absolute continuous case, coincides with the dimension of the support of $X$.
	Similar to \prettyref{rmk:dof}, the number of free real variables in $\text{span}(v)$ is $2n-2$, which is consistent with the information dimension characterization.
%	Low-distortion behavior $n-1 = \frac{1}{2} (2n - 1 - 1)$.
\end{remark}


%The proof is to relate the rate-distortion behavior of a random unit vector to that of a standard Gaussian vector.
\begin{proof}
Under the mean-square error distortion, the rate-distortion function for $\calCN(0,1)$ is given by
		\begin{equation}
		R(D) = \log^+ \frac{1}{D}, \quad D > 0.
	\label{eq:RDCN}
\end{equation}
		Let $W \sim \calCN(0,I_n)$. Then $W = X + i Y$, where $X,Y \, \iiddistr \calN(0, \frac{1}{2}I_n)$. As a consequence of \prettyref{eq:RDCN}, for any $a > 0$,
		\begin{equation}
	\inf_{P_{\hW|W}:\, \Expect \|\hW-W\|_2^2 \leq n a} I(W;\hat{W}) \geq n \log^+ \frac{1}{a}.
	\label{eq:IWW}
\end{equation}
			Put $L = \|W\|_2$ and $v=\frac{W}{L}$. Since $ \frac{1}{L} (X,Y)$ is uniformly distributed on the unit sphere in $\reals^{2n}$, it is straightforward to verify that $v$ is uniform on the complex unit sphere $\bbS^{2n-1}$.


Fix $0 < D < 2$.
Fix any probability transition kernel $P_{\hv\hv^*|vv^*}$ from $E_n$ to itself, such that $\Expect{\|vv^*-\hv\hv^*\|_2^2} \leq D$.
Since $\|v\| = \|\hv\| = 1$, we have $\|vv-\hv\hv^*\|_2^2 = 2 - 2 |\Iprod{v}{\hv}|^2$ and $\Expect |\Iprod{v}{\hv}|^2 \geq 1 - \frac{D}{2}$.
Let $\Iprod{v}{\hv} = |\Iprod{v}{\hv}| \exp(i \phi)$ with $\phi \in [0,2\pi)$. Let $m \in \naturals$ to be optimized later. Denote the uniformly quantized version of $\phi$ by $\phi_m \triangleq \lfloor \frac{m\phi}{2\pi}\rfloor \frac{2\pi}{m}$, which satisfies $\phi_m \leq \phi < \phi_m + \frac{2\pi}{m}$.
Set $\tv = \hv \exp(i\phi_m)$. Then
\[
\Real(\Iprod{v}{\tv})
= |\Iprod{v}{\hv}| \cos(\phi-\phi_m) \geq  \pth{1 - \frac{2\pi^2}{m^2}} |\Iprod{v}{\hv}|,
\]
where the last inequality follows from $1-\cos(\theta)\leq \frac{\theta^2}{2}$ for all $\theta\in \reals$. Since $\Expect |\Iprod{v}{\hv}| \geq \Expect |\Iprod{v}{\hv}|^2 \geq 1 - \frac{D}{2}$, setting $m = \ceil{\frac{2\pi}{\sqrt{D}}}$ yields

\begin{equation}
\Expect \|v-\tv\|_2^2  = 2 - 2 \Expect \, \Real(\Iprod{v}{\tv}) \leq 2 - 2\pth{1 - \frac{D}{2}}^2 \leq 2D.
	\label{eq:tv}
\end{equation}

Now we use $P_{\tv|v}$ to design a lossy compressor for the standard Gaussian vector. Fix a transition kernel $P_{\tL|L}$ to be specified later
%Let $k\in \naturals$ to be specified later. Let $\tL= \frac{\floor{k L}}{k}$ denote the quantized version of $L$
and set $\tW = \tL \tv$.
%To this end, let $U$ be uniformly distribution on $[0,1]$ and independent of $\{W,\tv\}$. Set $G = \|W\|^2 - n D U$.
The dependence diagram for all random variables is as follows:
\[
%\begin{tikzcd}
%v \arrow{rd} \arrow{r} 	& \hv \arrow{r} \arrow{d} & \tv								& L \arrow{r} & \tL \\
%												& \phi \arrow{r}					&  \phi_m \arrow{u} & 								& %U \arrow{u}
%\end{tikzcd}
\begin{tikzcd}
L	\arrow{r}							& \tL	\arrow{r}						& \tW 							& \\		
v \arrow{rd} \arrow{r} 	& \hv \arrow{r} \arrow{d} & \tv	\arrow{u} 		& \\
												& \phi \arrow{r}					&  \phi_m \arrow{u} &
\end{tikzcd}
\]
which implies that
\begin{align}
I(W;\tW)
= & ~ I(v, L;\tv,\tL) = I(L;\tL)+I(v;\tv) \leq I(L;\tL)+I(v;\hv \exp(i\phi_m))	\nonumber \\
\leq & ~ I(v;\hv) + I(L;\tL) + H(\phi_m).	\label{eq:Ivv}
\end{align}
Since $\|W-\tW\| \leq L \|v-\tv\| + |L-\tL|$ and $L \indep \{v,\tv\}$, we have $\Expect \|W-\tW\|^2 \leq 2 \, \Expect L^2 \, \Expect \|v-\tv\|^2 + 2 \, \Expect |L-\tL|^2$.
Note that $2L^2$ is distributed according to the $\chi^2$-distribution with $2n$ degress of freedom, denoted by $\chi^2_{2 n}$, hence $\Expect L^2 = n$.
Moreover, $\Expect L = \frac{\Gamma(n + \frac{1}{2})}{\Gamma(n)}$ and $\frac{\Gamma(n + \frac{1}{2})}{\Gamma(n) \sqrt{n-1}} \geq 1$ for any $n \geq 2$.  Therefore $\var L \leq 1$.
By \cite[Theorem 4.3.3]{berger}, the rate-distortion function of $L$ is majorized by that of the standard normal distribution, \ie,
\[
\min_{P_{\tL|L}: \Expect (\tL-L)^2 \leq a} I(L;\tL) \leq \frac{1}{2} \log^+ \frac{1}{a}, \quad a > 0.
\]
Therefore there exists $P_{\tL|L}$ such that $\Expect (\tL-L)^2 \leq nD$ and $I(L;\tL) \leq \frac{1}{2} \log^+ \frac{1}{nD}$. Therefore
\[
\Expect \|W-\tW\|^2 \leq 6nD.
\]
In view of \prettyref{eq:IWW} and \prettyref{eq:Ivv}, we have
\[
I(v;\hv) \geq n \log^+ \frac{1}{6D} - H(\phi_m) - \frac{1}{2} \log^+ \frac{1}{nD}.
\]
Note that $\phi_m$ is a random variable which takes no more than $m$ values, hence $H(\phi_m) \leq \log m \leq \log (1+\frac{2\pi}{\sqrt{D}})$. Therefore
\[
I(v;\hv) \geq n \log^+ \frac{1}{6D} - \log \Big(1+\frac{2\pi}{\sqrt{D}}\Big) -\frac{1}{2} \log^+ \frac{1}{nD} \geq (n-1) \log^+ \frac{1}{6D} - 3.5.
\]
where we used $n \geq 2$ and $D < 2$.
\end{proof}

\iffalse
By definition, $(L-\tL)^2 \leq \frac{1}{k^2}$.
Now setting $k = \ceil{\frac{1}{\sqrt{nD}}}$ and in view of \prettyref{eq:tv}, we have

Invoking \prettyref{lmm:quant}, we have $H(\tL) \leq 3 \log 2 + \frac{1}{2} \log \frac{\pi \eexp}{6} + \frac{1}{2} \log (1 + k^2 \var L)$. Note that $\Expect L = \frac{\Gamma(n + \frac{1}{2})}{\Gamma(n)}$ and $\frac{\Gamma(n + \frac{1}{2})}{\Gamma(n) \sqrt{n-1}} \geq 1$ for any $n \geq 2$.  Therefore $\var L \leq 1$. Moreover, $k^2 \leq 2(1+\frac{1}{nD})$. Consequently,
\[
H(\tL) \leq 4 \log 2 + \frac{1}{2} \log \frac{\pi \eexp}{6} + \frac{1}{2} \log (1+\frac{1}{nD}).
\]



\begin{lemma}
Let $X$ be a real-valued random variable with $\Expect X^2 < \infty$. Denote by $\quant{X}_k = \frac{\floor{k Y}}{k}$ the quantized version of $X$. Then
\begin{equation}
H(\quant{X}_k) \leq 3 \log 2 + \frac{1}{2} \log \frac{\pi \eexp}{6} + \frac{1}{2} \log (1 + k^2 \var X).
	\label{eq:quant}
\end{equation}
	\label{lmm:quant}
\end{lemma}
\begin{proof}
Define $g(X,\epsilon) \triangleq \Expect[ \log \frac{1}{P_{X}(B(X,\epsilon))}]$. By \cite[Eq. (294) and (296)]{renyi.ITtrans} (or \cite[Lemma 2.3]{peres.conformal}), for any $k \in \naturals$, $H(\quant{X}_k) \leq  g(X, 1/k) + 3$.
Let $U$ be uniformly distributed on $[-\sqrt{3},\sqrt{3}]$ and independent of $X$.
Then $U$ has zero mean and \emph{unit} variance. Hence \cite{Ihara78}
\begin{equation}
%	I(X; \qsnr X + \Phi_U) \leq I(X; \qsnr X + U) \leq I(X; \qsnr X + \Phi_U) + D(U \, || \, \Phi_U),
I(X; a X + U) \leq I(X; a X + Z) + \frac{1}{2} \log \frac{\pi \eexp}{6},
	\label{eq:phiu}
\end{equation}
where $Z \sim \calN(0,1)$ is independent of $X$.
Then
\begin{align}
I(X; X + \epsilon U)
= & ~ D(P_{Y|X} \, || \, P_Y \, | \, P_X)\\
%= & ~ h(Y) + \frac{1}{2}\log \snr - h(U) \\
= & ~ \expect{\log \frac{1}{P_X(B(X + \epsilon U,\sqrt{3}\epsilon))}} \\
\geq & ~ \expect{\log \frac{1}{P_X(B(X,2 \sqrt{3}\epsilon))}}, \label{eq:lb}
\end{align}	
\end{proof}
\fi


==> initrs_old.tex <==
In the row-sparse case ($s_2 = n_2$), the support estimate for $v$ is trivially given as $\widehat{J}_2 = [n_2]$.
The assumptions of Theorem~\ref{thm:pgrip_init_rs} imply
\begin{equation}
\delta+\nu+\delta\nu < \min\left( \frac{\sin \omega_{\sup} \norm{u}_\infty}{1 + \sin \omega_{\sup}}, \frac{\norm{u}_\infty}{2} \right)
\label{eq:proof:thm:pgrip_init_rs:cond}
\end{equation}

Let $j_0 \in [n_1]$ denote the index of the largest entry of $u$ in magnitude, i.e.,
\[
j_0 \triangleq \argmax_{j \in [n_1]} |[u]_j|.
\]
Then, $|[u]_{j_0}| = \norm{\Pi_{\{j_0\}} u}_2 = \norm{u}_\infty$.

Since (\ref{eq:proof:thm:pgrip_init_rs:cond}) implies
\begin{equation}
2\delta + 2(1+\delta)\nu < \norm{u}_\infty,
\end{equation}
by Lemma~\ref{lemma:est_supp_dthres} with $\widetilde{J}_1 = \{j_0\}$,
it follows that $j_0 \in \widehat{J}_1$; hence,
\begin{equation}
\norm{\Pi_{\widehat{J}_1} u}_2 \geq \norm{u}_\infty.
\label{eq:proof:thm:pgrip_init_rs:bnd}
\end{equation}

On the other hands, since $\Pi_{\widehat{J}_2}^\perp v = 0$, by Lemma~\ref{lemma:init_w_good_est_supp2},
we get a sufficient condition for (\ref{eq:conv_spf_initcond}) given by
\begin{equation}
\delta + (1+\delta) \nu < \frac{\sin \omega_{\sup} \norm{\Pi_{\widehat{J}_1} u}_2}{1 + \sin \omega_{\sup}}.
\label{eq:proof:thm:pgrip_init_rs:cond2}
\end{equation}

Finally, note that (\ref{eq:proof:thm:pgrip_init_rs:cond}) also implies (\ref{eq:proof:thm:pgrip_init_rs:cond2})
since (\ref{eq:proof:thm:pgrip_init_rs:bnd}) holds.


==> nonzeros.tex <==
\begin{lemma}[Exponentially decaying nonzero magnitudes]
\label{lemma:lindecay}
Suppose that the magnitudes of the nonzero entries in an $s$-sparse $u \in \bbS^{n-1}$ decay exponentially with a constant $\rho \in (0,1)$.
Then, there exists $\widetilde{J} \subset [n]$ such that
\[
\norm{\Pi_{\widetilde{J}} u}_2 \geq 1-\epsilon
\]
and
\begin{align*}
|[u]_j| \geq \sqrt{(1-\rho^2) \epsilon}, \quad \forall j \in \widetilde{J}.
\end{align*}
\end{lemma}

\begin{proof}%[Proof of Lemma~\ref{lemma:lindecay}]
Without loss of generality, we assume that the magnitudes are sorted in decreasing order.
Then,
\[
|[u]_k| = \sqrt{\frac{1-\rho^2}{1-\rho^{2s}}} \cdot \rho^{k-1}
\]
for $k = 1,\ldots,s$.

Let $k_0 \in [s]$ satisfy $\rho^{2 k_0} < \epsilon$ and $\rho^{2 (k_0-1)} \geq \epsilon$.
(Such $k_0$ exists if $s$ is large enough.)
Then,
\[
\sum_{k=k_0+1}^s \frac{1-\rho^2}{1-\rho^{2s}} \cdot \rho^{2k}
= \frac{1-\rho^{2(s-k_0)}}{1-\rho^{2s}} \cdot \rho^{2(k_0+1)}
\leq \rho^{2 k_0} \leq \epsilon.
\]

Therefore, for all $k \leq k_0$,
\[
|[u]_j| \geq \sqrt{\frac{1-\rho^2}{1-\rho^{2s}}} \cdot \rho^{k_0-1} \geq \sqrt{1-\rho^2} \cdot \rho^{k_0-1}.
\]
\end{proof}%[Proof of Lemma~\ref{lemma:lindecay}]

Next, we consider the power-law decay case.
Suppose that the magnitudes of an $s$-sparse $u \in \bbS^{n-1}$ are sorted in decreasing order so that
\[
|[u]_k| = \left(\sum_{k=1}^s k^{-2 \alpha}\right)^{-1/2} k^{-\alpha}, \quad \forall k \in [s].
\]
for some $\alpha > 0.5$.
Then,
\[
\sum_{k=1}^{m-1} k^{-2 \alpha} \approx \int_1^{m+1} t^{-2\alpha} dt = \frac{1-m^{1-2\alpha}}{2\alpha-1}
\]

Suppose that
\[
\sum_{k=1}^{m-1} k^{-2 \alpha} \geq (1-\epsilon)^2 \sum_{k=1}^s k^{-2 \alpha},
\]
which is approximated as
\[
\frac{1-m^{1-2\alpha}}{1-s^{1-2\alpha}} \geq (1-\epsilon)^2.
\]
Then, it is implied that
\[
\left(\sum_{k=1}^s k^{-2 \alpha}\right)^{-1/2} m^{-\alpha} \geq
\frac{\left(1 - (1-\epsilon)^2 [1 - s^{1-2\alpha}]\right)^{\frac{\alpha}{2\alpha-1}}}{(1-s^{1-2\alpha})^{1/2}} (2\alpha-1)^{1/2}
\]
In particular, when $\alpha = 1$,
\[
|[u]_m| \geq \frac{s}{s-1} - (1-\epsilon)^2.
\]



==> pgdspf.tex <==
Almost the same, only slight changes...

\begin{lemma}[Initialization given a good estimate of support pair]
\label{lemma:init_w_good_est_supp2}
Suppose that $\widehat{J}_1 \subset \{1,\ldots,n_1\}$ with $|\widehat{J}_1| \leq 2s_1$
and $\widehat{J}_2 \subset \{1,\ldots,n_2\}$ with $|\widehat{J}_2| \leq 2s_2$ satisfy
\begin{equation}
\fnorm{\Pi_{\widehat{J}_1} u v^* \Pi_{\widehat{J}_2}}^2 > 1-\epsilon.
\label{eq:lemma:init_w_good_est_supp2:condeps}
\end{equation}
Let $v_0 \in \bbC^{n_2}$ be obtained as the right singular vector of $\Pi_{\widehat{J}_1} [\A^*(b)] \Pi_{\widehat{J}_2}$ that corresponds to the largest singular value.
Then,
\[
\sin \phi_0 \leq
\frac{\delta + \sqrt{\epsilon} + (1+\delta) \nu}{1 - \delta - \sqrt{\epsilon} - (1+\delta) \nu}.
\]
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lemma:init_w_good_est_supp2}]
Let $M := X$.
Let $\widehat{M}$ denote the best rank-one approximation of $\Pi_{\widehat{J}_1} [\A^*(b)] \Pi_{\widehat{J}_2}$ in the spectral norm.
Let $\Delta := \Pi_{\widehat{J}_1} [\A^*(b)] \Pi_{\widehat{J}_2} - M$.
Then,
\begin{align*}
\norm{M + \Delta - \widehat{M}}
{} & = \norm{\Pi_{\widehat{J}_1} [\A^*(b)] \Pi_{\widehat{J}_2} - \widehat{M}} \\
{} & \leq \norm{ \underbrace{ \Pi_{\widehat{J}_1} [\A^*(b)] \Pi_{\widehat{J}_2} - X }_{ = \Delta } } \\
{} & = \norm{\Pi_{\widehat{J}_1} [(\A^* \A - \idm)(X)] \Pi_{\widehat{J}_2}
+ (X - \Pi_{\widehat{J}_1} X \Pi_{\widehat{J}_2}) + \Pi_{\widehat{J}} [\A^*(z)]} \\
{} & \leq \norm{\Pi_{\widehat{J}_1} [(\A^* \A - \idm)(X)] \Pi_{\widehat{J}_2}}
+ \fnorm{X - \Pi_{\widehat{J}_1} X \Pi_{\widehat{J}_2}} + \norm{\Pi_{\widehat{J}} [\A^*(z)]} \\
{} & \leq (\delta+\sqrt{\epsilon}) \fnorm{X} + \sqrt{1+\delta} \norm{z}_2.
\end{align*}

Note that $v_0$ is the right singular vector of $\widehat{M}$.
Since $\R(M) = \R(X)$, by Lemma~\ref{lemma:sintheta}, we have
\begin{align*}
\sin (\R(X^*),\R(v_0))
{} & \leq \frac{\norm{\Delta}}{\norm{M} - \norm{M + \Delta - \widehat{M}}} \\
{} & \leq \frac{(\delta+\sqrt{\epsilon}) \fnorm{X} + \sqrt{1+\delta} \norm{z}_2}{(1-\delta-\sqrt{\epsilon}) \fnorm{X} - \sqrt{1+\delta} \norm{z}_2}.
\end{align*}

\end{proof}%[Proof of Lemma~\ref{lemma:init_w_good_est_supp2}]

Next two lemmata hold without changing the corresponding lemmata in the previous section.

\begin{lemma}[Estimation of partial support by DSPCA]
\label{lemma:est_supp_dspca}
Let $\widehat{J}_1 \subset \{1,\ldots,n_1\}$ and $\widehat{J}_2 \subset \{1,\ldots,n_2\}$ be given by (\ref{eq:initbydspca}). 
Then,
\[
\fnorm{\Pi_{\widehat{J}_1} u v^* \Pi_{\widehat{J}_2}}
\geq \sin \left[
\sin^{-1} \left( \frac{1 - \delta - 2 (1+\delta) \nu}{\sqrt{\delta^2 + (1+\delta)^2}} \right)
- \sin^{-1} \left( \frac{\delta}{\sqrt{\delta^2 + (1+\delta)^2}} \right) \right].
\]
\end{lemma}

$\delta \leq 0.036$ and $\nu \leq 0.01$

\begin{lemma}
\label{lemma:est_supp_jthres}
Let $\widehat{J}_1 \subset \{1,\ldots,n_1\}$ and $\widehat{J}_2 \subset \{1,\ldots,n_2\}$ be given by (\ref{eq:initbyjthres}).
Suppose that
\[
\delta < \frac{\chi_\epsilon(u,v) - \nu}{2 + 2 \nu}.
\]
Then, 
\begin{equation}
\fnorm{\Pi_{\widehat{J}_1} u v^* \Pi_{\widehat{J}_2}}^2 > 1-\epsilon.
\label{eq:lemma:est_supp_jthres:res}
\end{equation}
\end{lemma}

$\delta \leq 0.083$, $\rho \leq 0.088$, $\nu \leq 0.01$



==> pgpf.tex <==
As a side result, Lemma~\ref{lemma:update_theta} leads to performance guarantees for PF
that improve on the previous results \cite{JaiNS2012} in terms of constants for threshold on $\delta$ and $\nu$.

\begin{theorem}[{RIP-guarantee for PF; slight improvement on a previous analysis \cite{JaiNS2012}}]
\label{thm:pgpfrip}
Suppose that $\A$ satisfies the rank-2 RIP with isometry constant $\delta \leq 0.3$ and $X$ is a rank-one matrix.
Let $b = \A(X) + z$, where $\norm{z}_2 \leq 0.08 \norm{\A(X)}_2$.
Then, PF converges linearly to an estimate $\hat{X}$ of $X$ that satisfies
\[
\frac{\fnorm{\hat{X} - X}}{\fnorm{X}} \leq 4.77 \frac{\norm{z}_2}{\norm{\A(X)}_2}.
\]
\end{theorem}

Compared to the previous result on the recovery by PF \cite{JaiNS2012},
Theorem~\ref{thm:pgpfrip} requires a larger threshold on the isometry constant.
Since an i.i.d. Gaussian measurement operator satisfies the rank-$r$ RIP
with $O(r(n_1+n_2)\log[\max(n_1,n_2)])$ measurements \cite{RecFP2010},
the recovery of a rank-one matrix by PF from $O(r(n_1+n_2)\log[\max(n_1,n_2)])$ measurements is guaranteed.
Comparing this to Theorem~\ref{thm:pgspfiidG}, we note that
when the unknown matrix is a row-sparse rank-one matrix,
the recovery by SPF is guaranteed by a significantly less demanding condition.

\begin{theorem}[RIP-guarantee for PF: conditioned on a good initialization]
\label{thm:conv_pf}
Suppose that $\A$ satisfies the rank-2 RIP with isometry constant $\delta$, and that $X = \lambda u v^*$.
Let $b = \A(X) + z$ and $\nu$ be defined in (\ref{eq:defnu}).
If the initialization $v_0$ satisfies
\begin{equation}
\frac{|v_0^* v|}{\norm{v_0}_2 \norm{v}_2} > \inf_{\omega \in [0, \pi/2)} \left\{ \cos \omega : \omega \geq \sin^{-1} \left( \frac{\delta \tan \omega + (1+\delta) \nu \sec \omega}{1-\delta} \right) \right\}.
\label{eq:conv_pf_initcond}
\end{equation}
then SPF produces $(X_t)_{t \in \bbN}$ satisfying
\begin{equation}
\limsup_{t \to \infty} \frac{\norm{X - X_t}_{\mathrm{F}}}{\norm{X}_{\mathrm{F}}} \leq C \nu.
\label{eq:conv_pf_res}
\end{equation}
for a universal constant $C$ that only depends on $\delta$ and $\nu$.
Furthermore, the convergence is superlinear.
\end{theorem}

Since the proof of Theorem~\ref{thm:conv_pf} is almost identical to that of Theorem~\ref{thm:conv_spf} except
that $C_\delta^{\text{\rm HTP}}$ is replaced by $(1-\delta)^{-1}$, we omit the derivation of Theorem~\ref{thm:conv_pf}.
When $\delta \leq 0.3$ and $\nu \leq 0.08$, the noise amplification in Theorem~\ref{thm:conv_spf} is explicitly bounded by $C \leq 4.77$.

Unlike SPF, the initialization of PF is done by singular value decomposition of the proxy matrix $\A^*(b)$ without involving any support estimation, which has been proposed and analyzed by Jain et al. \cite{JaiNS2012}.
Using the non-Hermitian $\sin \theta$ theorem \cite{Wed1972perturbation} (Lemma~\ref{lemma:sintheta}),
we present a slightly improved analysis of this initialization, which also leads to the improvement in constants in Theorem~\ref{thm:pgpfrip}.

\begin{lemma}[Initialization]
\label{lemma:init_pf}
Let $v_0$ be obtained as the leading right singular vector of $\A^*(b)$.
Then,
\[
\sin \phi_0 \leq
\frac{\delta + (1+\delta) \nu}{1 - \delta - (1+\delta) \nu}.
\]
\end{lemma}

\begin{proof}%[Proof of Lemma~\ref{lemma:init_pf}]
Let $M \triangleq X$.
Let $\widehat{M}$ denote the best rank-one approximation of $\A^*(b)$ in the spectral norm.
Let $\Delta \triangleq [\A^*(b)] - M$.
Then,
\begin{align*}
\norm{M + \Delta - \widehat{M}}
{} & = \norm{[\A^*(b)] - \widehat{M}} \\
{} & \leq \norm{ \underbrace{ [\A^*(b)] - X }_{ = \Delta } } \\
{} & \leq \norm{(\A^* \A - \idm)(X)} + \norm{\A^*(z)} \\
{} & \leq \delta \fnorm{X} + \sqrt{1+\delta} \norm{z}_2.
\end{align*}

By Lemma~\ref{lemma:sintheta}, we have
\begin{align*}
\sin (\R(X^*),\R(v_0))
{} & \leq \frac{\norm{\Delta}}{\norm{M} - \norm{M + \Delta - \widehat{M}}} \\
{} & \leq \frac{\delta \fnorm{X} + \sqrt{1+\delta} \norm{z}_2}{\fnorm{X} - \delta \fnorm{X} - \sqrt{1+\delta} \norm{z}_2}.
\end{align*}
Applying (\ref{eq:nuineq}) to this result, we get the assertion in Lemma~\ref{lemma:init_w_good_est_supp}.
\end{proof}%[Proof of Lemma~\ref{lemma:init_pf}]

Combining Theorem~\ref{thm:conv_pf} and Lemma~\ref{lemma:init_pf} yields Theorem~\ref{thm:pgpfrip}.



==> ripiidG.tex <==
\begin{theorem}
\label{thm:ripiidG}
Let $\A: \mathbb{C}^{n \times d} \to \mathbb{C}^m$ be an i.i.d. Gaussian operator.
\[
[\A(X)]_k = \frac{1}{\sqrt{m}} \langle \xi_k, X \rangle, \quad k = 1,\ldots,m
\]
where $\xi_k \in \mathbb{C}^{n \times d}$ has the standard i.i.d. Gaussian entries.
If
\[
m \geq c_1 r(s+d+1) \ln\left(\frac{n}{s}\right)
\]
then with probability at least $1 - \exp(-c_2 m)$
\begin{equation*}
(1-\delta) \norm{X}_{\mathrm{F}}^2 \leq \norm{\A(X)}_2^2 \leq (1+\delta) \norm{X}_{\mathrm{F}}^2
\end{equation*}
for all $X \in \bbC^{n \times d}$ such that $\rank(X) \leq r$ and $\norm{X}_{0,2} \leq s$, 
where $c_1$ and $c_2$ are universal constants that depend on $\delta$.
\end{theorem}

\begin{theorem}
\label{thm:ripiidGds}
Let $\A: \mathbb{C}^{n \times d} \to \mathbb{C}^m$ be an i.i.d. Gaussian operator.
\[
[\A(X)]_k = \frac{1}{\sqrt{m}} \langle \xi_k, X \rangle, \quad k = 1,\ldots,m
\]
where $\xi_k \in \mathbb{C}^{n \times d}$ has the standard i.i.d. Gaussian entries.
If
\[
m \geq c_3 r(s_{\text{row}}+s_{\text{col}}+1) \ln \left[ \max\left(\frac{n}{s_{\text{row}}}, \frac{d}{s_{\text{col}}}\right) \right]
\]
then with probability at least $1 - \exp(-c_4 m)$
\begin{equation*}
(1-\delta) \norm{X}_{\mathrm{F}}^2 \leq \norm{\A(X)}_2^2 \leq (1+\delta) \norm{X}_{\mathrm{F}}^2
\end{equation*}
for all $X \in \bbC^{n \times d}$ such that $\rank(X) \leq r$, $\norm{X}_{0,2} \leq s_{\text{row}}$, and $\norm{X^*}_{0,2} \leq s_{\text{col}}$, 
where $c_1$ and $c_2$ are universal constants that depend on $\delta$.
\end{theorem}

The proofs of Theorem~\ref{thm:ripiidG} and Theorem~\ref{thm:ripiidGds} are rather straightforward; hence, we only provide a sketch. 
It follows from the standard volume argument and the exponential concentration of the i.i.d. Gaussian linear operator \cite{BarDdVW2008simple}. 
The only difference from the derivation of the standard RIP \cite{BarDdVW2008simple} is the use of the net of rank-$r$ matrices, the cardinality of which is bounded according to the following lemma. 

\begin{lemma}[$\epsilon$-net of rank-$r$ matrices \cite{CanPla2011oracle}]
Let $\mathcal{S} = \{ X \in \mathbb{C}^{n \times d} :~ \text{rank}(X) \leq r,~ \norm{X}_F = 1 \}$.
There exists a subset $\mathcal{S}_\epsilon$ of $\mathcal{S}$ such that
\[
\sup_{X \in \mathcal{S}} \inf_{\hat{X} \in \mathcal{S}_\epsilon} \norm{X - \hat{X}}_F \leq \epsilon
\]
and
\[
|\mathcal{S}_\epsilon| \leq \left(\frac{9}{\epsilon}\right)^{(n+d+1)r}.
\]
\end{lemma}


==> unit-RD.tex <==
\begin{lemma}
	Let $v$ be uniformly distributed on the unit sphere in $\complex^{n}$. Then for any $n \geq 2$ and any $0 < D < 2$,
	\begin{align}
	\inf_{P_{\hv|v}: \Expect \|v-\hv\|_2^2 \leq D} I(v;\hv)  \geq & ~ 	n \log^+ \frac{1}{D+\frac{D^2}{4} + \frac{1}{n}\big(1-\frac{D}{2}\big)^2}, 	\label{eq:RDv}
\end{align}
where $\log^+ \triangleq \max\{\log, 0\}$.
	\label{lmm:RDv}
\end{lemma}
\begin{proof}
		Under the mean-square error distortion, the rate-distortion function for $\calCN(0,1)$ is given by
		\begin{equation}
		R(D) = \log^+ \frac{1}{D}, \quad D > 0.
	\label{eq:RDCN}
\end{equation}
		Let $W \sim \calCN(0,I_n)$. Then $W = X + i Y$, where $X,Y \, \iiddistr \calN(0, \frac{1}{2}I_n)$. As a consequence of \prettyref{eq:RDCN}, for any $a \in (0,1)$,
		\begin{equation}
	\inf_{P_{\hW|W}:\, \Expect \|\hW-W\|_2^2 \leq n a} I(W;\hat{W}) \geq n \log \frac{1}{a}.
	\label{eq:IWW}
\end{equation}
			Put $v=\frac{W}{\norm{W}_2}$. Since $ \frac{1}{\|W\|_2} (X,Y)$ is uniformly distributed on the unit sphere in $\reals^{2n}$, it is straightforward to verify that $v$ is uniform on the unit sphere in $\complex^{n}$, which we denote by $\bbS^{2n-1}$. % Hence $v \eqdistr w$.
			
Fix any probability transition kernel $P_{\hv|v}$ from $\bbS^{2n-1}$ to itself, such that $\Expect{\|v-\hv\|_2^2} \leq D$.
%, we define a probability distribution $P_{\hw}$ as the output distribution of $P_{\hv|v}$ when the input is $w$. 
%		Set $\hZ = \norm{Z} \hv$. Then $\Expect \|Z-\hZ\|_2^2 = \Expect \norm{Z}_2^2 \|v-\hv\|_2^2 = \Expect \norm{Z}_2^2 \Expect \|v-\hv\|_2^2 = 2n D$. As a consequence of \prettyref{eq:RDCN}, 
%		\[
%		I(Z;\hZ) \geq n \log \frac{1}{D}
%		\]
	Set $\hW = \alpha \hv$ where $\alpha$ is a constant to be specified later. Since $\norm{W} \indep (v,\hv)$, we have 
	$\Expect \|W-\hW\|_2^2 = \alpha^2 + \Expect \|W\|^2  - 2 \alpha \Expect \|W\| \Expect \iprod{v}{\hv}$, where $2 \|W\|^2$ is distributed according to the $\chi^2$-distribution with $2n$ degress of freedom, denoted by $\chi^2_{2 n}$. Then $\Expect \|W\|^2 = n$ and $\Expect \|W\| = \frac{\Gamma(n + \frac{1}{2})}{\Gamma(n)}$. 
	Note that $\frac{\Gamma(n + \frac{1}{2})}{\Gamma(n) \sqrt{n-1}} \geq 1$ for any $n \geq 2$.  
	Choosing $\alpha = \Expect \|W\| \Expect \iprod{v}{\hv}$ yields 
	$\Expect \|Z-\hZ\|_2^2 = \Expect \|W\|^2 - (\Expect \|W\|)^2 |\Expect \iprod{v}{\hv}|^2 \leq n - (n-1)(1-\frac{D}{2})^2 = n (D+\frac{D^2}{4}) + (1-\frac{D}{2})^2$,
	where we have used $\Expect \iprod{v}{\hv} = 1 - \frac{1}{2} \Expect{\|v-\hv\|_2^2} \geq  1 - \frac{D}{2}$.	
	As a consequence of \prettyref{eq:RDCN}, 
		\[
		I(W;\hW) \geq n \log^+ \frac{1}{D+\frac{D^2}{4} + \frac{1}{n}\big(1-\frac{D}{2}\big)^2}
		\]
		Then \prettyref{eq:RDv} follows upon noting that $I(W;\hW) = I(v,\|W\|;\alpha \hv) = I(v;\alpha \hv)$ since $\norm{W} \indep (v,\hv)$.		
		
%		It remains to prove \prettyref{eq:RDvv}. 	 Given a matrix $A \in \reals^{n \times d}$, define $v_1(A) \in \bbS^{d-1}$ as the unit right singular vector that is closest to the coordinate vector $e_1$. The choice of $e_1$ is arbitrary to resolve ambiguity. Formally, if $A=UDV$ is the SVD of $A$ and $V_{*1}$ is the first column of $V$, then $v_1(A) = \exp(i \theta) V_{*1}$, where $\theta = \argmax_{\alpha \in [0,2\pi)} \|\exp(i \alpha) V_{*1} - e_1\|$.
%	 
%
%	Define $\tilde{v} \triangleq v_1(\hv\hv^*)$. Then $\tv\tv^*=\hv\hv^*$.
%%	$\tilde{v}= \exp(i \theta) \hv$ for some $\theta \in [0,2\pi)$. 
%
%
%%Since $\fnorm{uv^* - \hu\hv^*} \leq \sqrt{D}$ and $\rank(uv^* - \hu\hv^*)\leq 2$, we have
%Let $\hv^{\perp} = v - \iprod{v}{\hv}\hv$. Then $\hv^{\perp} \perp \hv$ and $\|\hv^{\perp}\|_2^2 = 1 - |\iprod{v}{\hv}|^2 = \frac{1}{2} \fnorm{vv^* - \hv\hv^*}^2$. Since $(uv^* - \hu\hv^*)\hv^{\perp} = \|\hv^{\perp}\|_2^2 u$, we have $\opnorm{uv^* - \hu\hv^*} \geq \|\hv^{\perp}\|_2 = \frac{1}{\sqrt{2}} \fnorm{vv^* - \hv\hv^*}$.
%In view of $\Expect \opnorm{uv^* - \hu\hv^*}^2 \leq \Expect \fnorm{uv^* - \hu\hv^*}^2 \leq D$, we have $\Expect \fnorm{vv^* - \hv\hv^*}^2 \leq 2 D$.
%
%	
%		Consider the following Markov chain: $v \to vv^* \to \hv\hv^* \to  \tilde{v}$.
%		
%		
%
%%		To this end, let $W \sim \calC\calN(0,I_n)$. Then $v \eqdistr \frac{W}{\|W\|_2}$.
		
\end{proof}
